Ferrers Dimension and Boxicity

This note explores the relation between the boxicity of undirected graphs and the Ferrers dimension of digraphs.

==> bibmr.tex <==
 Clipboard 
Home Help Support Mail \bib{MR2389609}{article}{
   author={Chandran, L. Sunil},
   author={Francis, Mathew C.},
   author={Sivadasan, Naveen},
   title={Boxicity and maximum degree},
   journal={J. Combin. Theory Ser. B},
   volume={98},
   date={2008},
   number={2},
   pages={443--445},
   issn={0095-8956},
   review={\MR{2389609}},
}
		\bib{MR2344136}{article}{
   author={Chandran, L. Sunil},
   author={Sivadasan, Naveen},
   title={Boxicity and treewidth},
   journal={J. Combin. Theory Ser. B},
   volume={97},
   date={2007},
   number={5},
   pages={733--744},
   issn={0095-8956},
   review={\MR{2344136 (2008f:05125)}},
}
		\bib{MR2335890}{article}{
   author={Rosgen, Bill},
   author={Stewart, Lorna},
   title={Complexity results on graphs with few cliques},
   journal={Discrete Math. Theor. Comput. Sci.},
   volume={9},
   date={2007},
   number={1},
   pages={127--135 (electronic)},
   issn={1365-8050},
   review={\MR{2335890 (2008f:05190)}},
}
		\bib{MR2255615}{article}{
   author={Bohra, Ankur},
   author={Chandran, L. Sunil},
   author={Raju, J. Krishnam},
   title={Boxicity of series-parallel graphs},
   journal={Discrete Math.},
   volume={306},
   date={2006},
   number={18},
   pages={2219--2221},
   issn={0012-365X},
   review={\MR{2255615}},
}
		\bib{MR2130594}{article}{
   author={Chandran, L. S.},
   author={Mannino, C.},
   author={Oriolo, G.},
   title={On the cubicity of certain graphs},
   journal={Inform. Process. Lett.},
   volume={94},
   date={2005},
   number={3},
   pages={113--118},
   issn={0020-0190},
   review={\MR{2130594 (2005j:05067)}},
}
		\bib{MR1821631}{article}{
   author={McKee, Terry A.},
   title={Clique representations and dimension-$k$ chordal graphs},
   journal={J. Combin. Math. Combin. Comput.},
   volume={36},
   date={2001},
   pages={139--148},
   issn={0835-3026},
   review={\MR{1821631 (2001m:05178)}},
}
		\bib{MR1985050}{article}{
   author={Chang, Yi-Wu},
   author={West, Douglas B.},
   title={Interval number and boxicity of directed graphs},
   conference={
      title={Combinatorics, graph theory, and algorithms, Vol. I, II
      (Kalamazoo, MI, 1996)},
   },
   book={
      publisher={New Issues Press, Kalamazoo, MI},
   },
   date={1999},
   pages={171--179},
   review={\MR{1985050}},
}
		\bib{MR1985033}{collection}{
   title={Combinatorics, graph theory, and algorithms. Vol. I, II},
   booktitle={Proceedings of the 8th Quadrennial International Conference on
   Graph Theory, Combinatorics, Algorithms, and Applications, dedicated to
   the memory of Paul Erd\H os, held at Western Michigan University,
   Kalamazoo, MI, June 3--7, 1996},
   editor={Alavi, Y.},
   editor={Lick, D. R.},
   editor={Schwenk, A.},
   publisher={New Issues Press, Kalamazoo, MI},
   date={1999},
   pages={Vol. I: xviii+443 pp.; Vol II: pp. i--xii and 445--882},
   isbn={0-932826-76-8},
   review={\MR{1985033 (2004a:05003)}},
}
		\bib{MR1289974}{article}{
   author={Kratochv{\'{\i}}l, Jan},
   author={Tuza, Zsolt},
   title={Intersection dimensions of graph classes},
   journal={Graphs Combin.},
   volume={10},
   date={1994},
   number={2},
   pages={159--168},
   issn={0911-0119},
   review={\MR{1289974 (95k:05174)}},
}
		\bib{MR1217740}{article}{
   author={Bellantoni, S.},
   author={Hartman, I. Ben-Arroyo},
   author={Przytycka, T.},
   author={Whitesides, S.},
   title={Grid intersection graphs and boxicity},
   note={Combinatorics and algorithms (Jerusalem, 1988)},
   journal={Discrete Math.},
   volume={114},
   date={1993},
   number={1-3},
   pages={41--49},
   issn={0012-365X},
   review={\MR{1217740 (94b:05058)}},
}
		\bib{MR1217735}{collection}{
   title={Combinatorics and algorithms},
   editor={Fraenkel, A. S.},
   editor={Alon, N.},
   editor={Golumbic, M. C.},
   editor={Shamir, E.},
   note={Papers from the French-Israeli Conference held in Jerusalem,
   November 13--17, 1988;
   Discrete Math. {\bf 114} (1993), no. 1-3},
   publisher={Elsevier Science B.V.},
   place={Amsterdam},
   date={1993},
   pages={i--viii and 1--446},
   issn={0012-365X},
   review={\MR{1217735 (93k:00032)}},
}
		\bib{MR1217396}{article}{
   author={McKee, Terry A.},
   author={Scheinerman, Edward R.},
   title={On the chordality of a graph},
   journal={J. Graph Theory},
   volume={17},
   date={1993},
   number={2},
   pages={221--232},
   issn={0364-9024},
   review={\MR{1217396 (94b:05161)}},
}
		\bib{MR1148932}{article}{
   author={Raychaudhuri, Arundhati},
   title={Edge clique graphs of some important classes of graphs},
   journal={Ars Combin.},
   volume={32},
   date={1991},
   pages={269--278},
   issn={0381-7032},
   review={\MR{1148932 (92i:05179)}},
}
		\bib{MR1054977}{article}{
   author={Quest, Martin},
   author={Wegner, Gerd},
   title={Characterization of the graphs with boxicity $\leq 2$},
   journal={Discrete Math.},
   volume={81},
   date={1990},
   number={2},
   pages={187--192},
   issn={0012-365X},
   review={\MR{1054977 (91c:05158)}},
}
		\bib{MR981229}{article}{
   author={Cozzens, Margaret Barry},
   author={Roberts, Fred S.},
   title={On dimensional properties of graphs},
   journal={Graphs Combin.},
   volume={5},
   date={1989},
   number={1},
   pages={29--46},
   issn={0911-0119},
   review={\MR{981229 (89m:05103)}},
}
		\bib{MR882619}{article}{
   author={Trotter, W. T., Jr.},
   author={West, Douglas B.},
   title={Poset boxicity of graphs},
   journal={Discrete Math.},
   volume={64},
   date={1987},
   number={1},
   pages={105--107},
   issn={0012-365X},
   review={\MR{882619 (88e:05104)}},
}
		\bib{MR797516}{article}{
   author={Steif, Jeffrey E.},
   title={The frame dimension and the complete overlap dimension of a graph},
   journal={J. Graph Theory},
   volume={9},
   date={1985},
   number={2},
   pages={285--299},
   issn={0364-9024},
   review={\MR{797516 (86i:05055)}},
}
		\bib{MR783770}{article}{
   author={Cozzens, Margaret B.},
   author={Roberts, Fred S.},
   title={On $k$-suitable sets of arrangements and the boxicity of a graph},
   journal={J. Combin. Inform. System Sci.},
   volume={9},
   date={1984},
   number={1},
   pages={14--24},
   issn={0250-9628},
   review={\MR{783770 (86i:05085)}},
}
		\bib{MR712922}{article}{
   author={Cozzens, Margaret B.},
   author={Roberts, Fred S.},
   title={Computing the boxicity of a graph by covering its complement by
   cointerval graphs},
   journal={Discrete Appl. Math.},
   volume={6},
   date={1983},
   number={3},
   pages={217--228},
   issn={0166-218X},
   review={\MR{712922 (85d:05142)}},
}
		\bib{MR666860}{article}{
   author={Yannakakis, Mihalis},
   title={The complexity of the partial order dimension problem},
   journal={SIAM J. Algebraic Discrete Methods},
   volume={3},
   date={1982},
   number={3},
   pages={351--358},
   issn={0196-5212},
   review={\MR{666860 (83m:68091)}},
}
		\bib{MR548629}{article}{
   author={Trotter, William T., Jr.},
   title={A characterization of Roberts' inequality for boxicity},
   journal={Discrete Math.},
   volume={28},
   date={1979},
   number={3},
   pages={303--313},
   issn={0012-365X},
   review={\MR{548629 (81a:05118)}},
}
		\bib{MR508050}{book}{
   author={Roberts, Fred S.},
   title={Graph theory and its applications to problems of society},
   series={CBMS-NSF Regional Conference Series in Applied Mathematics},
   volume={29},
   publisher={Society for Industrial and Applied Mathematics (SIAM)},
   place={Philadelphia, Pa.},
   date={1978},
   pages={v+122},
   review={\MR{508050 (80g:90036)}},
}
		\bib{MR0504054}{article}{
   author={Roberts, Fred S.},
   title={Food webs, competition graphs, and the boxicity of ecological
   phase space},
   conference={
      title={Theory and applications of graphs (Proc. Internat. Conf.,
      Western Mich. Univ., Kalamazoo, Mich., 1976)},
   },
   book={
      publisher={Springer},
      place={Berlin},
   },
   date={1978},
   pages={477--490. Lecture Notes in Math., Vol. 642},
   review={\MR{0504054 (58 \#20617)}},
}
		\bib{MR0472576}{book}{
   title={Theory and applications of graphs},
   series={Lecture Notes in Mathematics, Vol. 642},
   booktitle={Proceedings of the International Conference held at Western
   Michigan University, Kalamazoo, Mich., May 11--15, 1976},
   editor={Alavi, Yousef},
   editor={Lick, Don R.},
   publisher={Springer-Verlag},
   place={Berlin},
   date={1978},
   pages={xiv+635},
   isbn={3-540-08666-8},
   review={\MR{0472576 (57 \#12273)}},
}
		\bib{MR0252268}{article}{
   author={Roberts, Fred S.},
   title={On the boxicity and cubicity of a graph},
   conference={
      title={Recent Progress in Combinatorics (Proc. Third Waterloo Conf. on
      Combinatorics, 1968)},
   },
   book={
      publisher={Academic Press},
      place={New York},
   },
   date={1969},
   pages={301--310},
   review={\MR{0252268 (40 \#5489)}},
}
		\bib{MR0250896}{book}{
   title={Recent progress in combinatorics},
   series={Proceedings of the Third Waterloo Conference on Combinatorics,
   May 1968. Edited by W. T. Tutte},
   publisher={Academic Press},
   place={New York},
   date={1969},
   pages={xiv+347},
   review={\MR{0250896 (40 \#4128)}},
}
		Matches: 26 Show all results Select Page: Previous 1 2 Next © Copyright 2008, American Mathematical Society
Privacy Statement  American Mathematical Society
201 Charles Street
Providence, RI 02904-2294 
